Robust Individual Circadian Parameter Estimation for Biosignal-based Personalisation of Cancer Chronotherapy

In cancer treatment, chemotherapy is administered according a constant schedule. The chronotherapy approach, considering chronobiological drug delivery, adapts the chemotherapy profile to the circadian rhythms of the human organism. This reduces toxicity effects and at the same time enhances efficiency of chemotherapy. To personalize cancer treatment, chemotherapy profiles have to be further adapted to individual patients. Therefore, we present a new model to represent cycle phenomena in circadian rhythms. The model enables a more precise modelling of the underlying circadian rhythms. In comparison with the standard model, our model delivers better results in all defined quality indices. The new model can be used to adapt the chemotherapy profile efficiently to individual patients. The adaption to individual patients contributes to the aim of personalizing cancer therapy.

==> Content/Questions.tex <==
\section*{Questions}

\subsection*{General}

\begin{itemize}
\setlength{\itemsep}{40pt}
  \item Es heisst 2-4 Seiten. Ich wuerde schauen, dass ich so wenig und so
  abstrakt wie moeglich das Themas fasse. So 3 Seiten ca. Oder doch
  ausführlicher und die kompletten 4 Seiten ausreitzen?
  \item Generell wuerde ich so kurz wie moeglich. Waere des OK?
  \item Gibt es noch Arbeiten von bspw. der Arbeitsgruppe die zitiert werden
  sollten? Bspw. Paper ueber Gaitcad in Implementierung der Methoden, hier einen
  Satz?
  \item Generelle Schwerpunktausrichtung? Eher nur auf Estimating cycle
  phenomena in rhythms (example biorhythms). Oder auch Richtung Personalisierung
  von Chronotherapie.
  \item Was die Zitate betrifft, ich habe in der Arbeit alles in Bezug auf
  Chronotherapie und Krebs gemacht, deshalb hab ich fast nur Zitate in diese
  Richtung. Wuerde diese hier aber auch verwenden in generellem Kontext.
\end{itemize}

\vspace{1cm}


\subsection*{Introduction}

\begin{itemize}
\setlength{\itemsep}{40pt}
  \item Das Thema Krebs ganz herauslassen? Damit man Raum offen hat fuer spaeteres
  ausfuehrliches Anwendungspaper mit Bezug auf Chronotherapie? Oder erwähnen als
  ein Beispiel.
  \item Aus gleichem Grund Chronotherapie ganz rauslassen? Bzw nur Erwähnen,
  dass es Anwendungen gibt, wo Biosignale analysiert werden müsse (hier dann
  Bsp. Chronobiology bringen)
  \item Ich wuerde hier schon Bezug auf Biorythmen nehmen und diese als Beispiele
  anbringen, da dies genau in der Schilderung des Workshops verwendet wird.
  \newline \textit{``Biosignal analysis is a basic and exciting discipline in
  biomedical engi- neering. It contains the analysis of signals directly or indirectly
generated by an organism in order to extract relevant information
about the conformation''}
\item Bei Relevanz des Topic, Chronotherapy erwaehnen bzw. auch in Verbindung mit
Krebs (hier 2-3 Zitate von Levi) nur kurz in Nebensatz erwaehnen?
\end{itemize}

\vspace{1cm}



\subsection*{Methods}

\begin{itemize}
\setlength{\itemsep}{40pt}
  \item Wie ausfuehrlich das Methodenkapitel?
  \item Ich wuerde eher alles sehr kurz halten und nur anreisen. 
  \item Formeln wuerde ich ganz weglassen. Wenn man dies tut sollte man dann auf
  die Masterarbeit verweisen? Oder hier eine Formel bringen, welche die Extended
  Cosinor Funktion darstellt ohne auf die Herleitung einzugehen?
  \item Den Benchmark hier im Kontext miteinbringen oder weglassen? Wenn
  weglassen, wofuer sollte dieser dann noch verwendet werden?
  \item Bzw. geht auch den Benchmark nur zu erwaehnen und genauer darauf
  einzugehen? Falls ja, kann man diesen dann in der Evaluierung in der Results
  Section verwenden?
\end{itemize}

\vspace{1cm}



\subsection*{Results}

\begin{itemize}
\setlength{\itemsep}{40pt}
  \item Erwaehnen dass man die Methoden auch auf realen Datensaetzen angewandt
  hat? Hierbei Levi fragen? Ich glaube nicht dass wir hier diesbezueglich noch
  eine rechtzeitige Antwort bekommen.
  \item Wie Evaluierung der Methode (extended Cosinor analysis)?
  	\begin{itemize}
  		\item Anhand Bechmark? Dann Benchmark in Paper erwaehnen. In welche Tiefe
  		muss dieser dann beschrieben werden?
  		\item Anhand der Patiendaten. Kann man einfach sagen dass sind aufgenommene
  		Daten von Patienten ohne den Zusammenhang zu Krebs herauszustellen um
  		spaetere detailiertere Ausfuehrung von Chronotherpy nicht im Weg zu stehen?
	\end{itemize} 
\end{itemize}


